Load Restoration in Islanded Microgrids: Formulation and Solution Strategies

Adverse circumstances such as extreme weather events can cause significant disruptions to normal operation of electric distribution systems (DS), which includes isolating parts of the DS due to damaged transmission equipment. In this paper, we consider the problem of load restoration in a microgrid (MG) that is islanded from the upstream DS. The MG contains sources of distributed generation such as microturbines and renewable energy sources, as well as energy storage systems (ESS). We formulate the load restoration task as a non-convex optimization problem. This problem embodies the physics of the MG by leveraging a branch flow model, while incorporating salient phenomenon in islanded MGs such as the need for internal frequency regulation, and complementarity requirements arising in ESS operations. Since the formulated optimization problem is non-convex, we introduce a convex relaxation which can be solved through model predictive control as a baseline method. However, in order to solve the problem considering its full non-convexity, we leverage a policy-learning method called constrained policy optimization, a tailored version of which is used as our proposed algorithm. The aforementioned approaches, along with an additional deep learning method are compared through extensive simulations.

==> fig/mpc_scheme.tex <==
\usetikzlibrary{arrows,positioning}
%\input{arrowsnew}
\newcommand{\leftOffset}{3}
\newcommand{\baseLine}{0}
\newcommand{\baseOffset}{0.25}
\newcommand{\subx}{$2$}
\newcommand{\arrowhead}{open triangle 90}
\resizebox{\linewidth}{!}{
\begin{tikzpicture}
	\foreach \x in {1,2,3} {
		\ifthenelse{\equal{\x}{1}}{
			\draw[fill=orange] (\fpeval{\x+\leftOffset}, \fpeval{\baseLine+3.75+\baseOffset}) rectangle ++(1, 0.5) node[pos=.5]
			{$\mcal{X}_\fpeval{\x-0}$};}{
			\draw (\fpeval{\x+\leftOffset}, \fpeval{\baseLine+3.75+\baseOffset}) rectangle ++(1, 0.5) node[pos=.5]
			{$\mcal{X}_\fpeval{\x-0}$};
		}
	}
	\foreach \x in {2,3,4} {
		\ifthenelse{\equal{\x}{2}}{
			\draw[fill=orange] (\fpeval{\x+\leftOffset}, \fpeval{\baseLine+3+\baseOffset}) rectangle ++(1, 0.5) node[pos=.5] {$\mcal{X}_\fpeval{\x-0}$};}{
			\draw (\fpeval{\x+\leftOffset}, \fpeval{\baseLine+3+\baseOffset}) rectangle ++(1, 0.5) node[pos=.5] {$\mcal{X}_\fpeval{\x-0}$};
		}
	}
	\foreach \x in {3,4,5} {
		\ifthenelse{\equal{\x}{3}}{
			\draw[fill=orange] (\fpeval{\x+\leftOffset}, \fpeval{\baseLine+2.25+\baseOffset}) rectangle ++(1, 0.5) node[pos=.5] {$\mcal{X}_\fpeval{\x-0}$};}{
			\draw (\fpeval{\x+\leftOffset}, \fpeval{\baseLine+2.25+\baseOffset}) rectangle ++(1, 0.5) node[pos=.5] {$\mcal{X}_\fpeval{\x-0}$};
		}
	}
	\foreach \x in {6,7,8} {
		\renewcommand{\subx}{\ifthenelse{\equal{\x}{6}}{T}{
				\ifthenelse{\equal{\x}{7}}{T+H}{T+2H}}
		}
		\ifthenelse{\equal{\x}{6}}{
			\draw[fill=orange] (\fpeval{\x+\leftOffset}, \fpeval{\baseLine+0.75+\baseOffset}) rectangle ++(1, 0.5) node[pos=.5] {$\mcal{X}_{\subx}$};}{
			
			\ifthenelse{\equal{\x}{7}}{
				
				
				\draw (\fpeval{\x+\leftOffset}, \fpeval{\baseLine+0.75+\baseOffset}) rectangle ++(1, 0.5) node[pos=.5] {$\cdots$};
				
			}{
				
				\draw (\fpeval{\x+\leftOffset}, \fpeval{\baseLine+0.75+\baseOffset}) rectangle ++(1.3, 0.5) node[pos=.5] {$\mcal{X}_{T+H-1}$};
				
		}}
	}
	\foreach \x in {1,2,3,4,5,6} {
		\ifthenelse{\equal{\x}{1} \OR \equal{\x}{2} \OR \equal{\x}{3}}{
			\draw[fill=orange] (\fpeval{\x+\leftOffset}, \fpeval{\baseLine+0}) rectangle ++(1, 0.5) node[pos=.5] {$\mcal{X}_\fpeval{\x-0}$};
		}{\ifthenelse{\equal{\x}{4} \OR \equal{\x}{5}}{
				\draw[fill=orange] (\fpeval{\x+\leftOffset}, \fpeval{\baseLine+0}) rectangle ++(1, 0.5) node[pos=.5] {$\cdots$};
			}{
				\draw[fill=orange] (\fpeval{\x+\leftOffset}, \fpeval{\baseLine+0}) rectangle ++(1, 0.5) node[pos=.5] {$\mcal{X}_T$};
			}	
		}
	}
	% now draw arrows going down
	\draw [\arrowhead-](\fpeval{1.25+\leftOffset},\fpeval{0.5}) -- (\fpeval{1.25+\leftOffset},\fpeval{3.75+\baseOffset});
	\draw [\arrowhead-](\fpeval{2.25+\leftOffset},\fpeval{0.5}) -- (\fpeval{2.25+\leftOffset},\fpeval{3+\baseOffset});
	\draw [\arrowhead-](\fpeval{3.25+\leftOffset},\fpeval{0.5}) -- (\fpeval{3.25+\leftOffset},\fpeval{2.25+\baseOffset});
	\draw [\arrowhead-](\fpeval{6.5+\leftOffset},\fpeval{0.5}) -- (\fpeval{6.	5+\leftOffset},\fpeval{0.75+\baseOffset});
	% draw node arrows going up
	\draw [-](\fpeval{1.75+\leftOffset},\fpeval{0.5}) -- (\fpeval{1.75+\leftOffset},\fpeval{3+0.25+\baseOffset});
	\draw [-\arrowhead](\fpeval{1.75+\leftOffset},\fpeval{3+0.25+\baseOffset}) -- (\fpeval{2+\leftOffset},\fpeval{3+0.25+\baseOffset});
	\draw [-](\fpeval{2.75+\leftOffset},\fpeval{0.5}) -- (\fpeval{2.75+\leftOffset},\fpeval{2.25+0.25+\baseOffset});
	\draw [-\arrowhead](\fpeval{2.75+\leftOffset},\fpeval{2.25+0.25+\baseOffset}) -- (\fpeval{3+\leftOffset},\fpeval{2.25+0.25+\baseOffset});
	\draw [-](\fpeval{3.75+\leftOffset},\fpeval{0.5}) -- (\fpeval{3.75+\leftOffset},\fpeval{1.5+0.25+\baseOffset});
	\draw [-\arrowhead](\fpeval{3.75+\leftOffset},\fpeval{1.5+0.25+\baseOffset}) -- (\fpeval{4+\leftOffset},\fpeval{1.5+0.25+\baseOffset});
	\draw [-](\fpeval{5.75+\leftOffset},\fpeval{0.5}) -- (\fpeval{5.75+\leftOffset},\fpeval{0.75+0.25+\baseOffset});
	\draw [-\arrowhead](\fpeval{5.75+\leftOffset},\fpeval{0.75+0.25+\baseOffset}) -- (\fpeval{6+\leftOffset},\fpeval{0.75+0.25+\baseOffset});
	% nodes
	\node[] (topa) at (\fpeval{\leftOffset+1},\fpeval{3.75+0.25}) {};
	\node[] (topb) at (\fpeval{\leftOffset+1},\fpeval{3+0.25}) {};
	\node[] (topc) at (\fpeval{\leftOffset+1},\fpeval{2.25+0.25}) {};
	\node[] (topd) at (\fpeval{\leftOffset+1},\fpeval{0.75+0.25}) {};
	\node[] (tope) at (\fpeval{\leftOffset+1},\fpeval{0.25}) {};
	% texts
	\node[draw,left = 0cm of topa,align=left] at (\leftOffset,\fpeval{3.75+0.5}) {\textbf{Subproblem $1$}};
	\node[draw,left = 0cm of topb,align=left] at (\leftOffset,\fpeval{3+0.5}) {\textbf{Subproblem $2$}};
	\node[draw,left = 0cm of topc,align=left] at (\leftOffset,\fpeval{2.25+0.5}) {\textbf{Subproblem $3$}};
	\node[draw,left = 0cm of topd,align=left] at (\leftOffset,\fpeval{0.75+0.5}) {\textbf{Subproblem $T$}};
	\node[draw,left = 0cm of tope,align=left] at (\leftOffset,\fpeval{0.25}) {\textbf{MPC Solution}};
	% upper labels
	\node[] (topf) at (\fpeval{\leftOffset+1},\fpeval{4.5+0.25}) {};
	\node[left = 0cm of topf,align=left] at (\leftOffset,\fpeval{4.5+0.5}) {\emph{Time steps} $\rightarrow$};
	\node[draw] at (\fpeval{\leftOffset+1.5},\fpeval{4.5+0.5}) {$t=1$};	
	\node[draw] at (\fpeval{\leftOffset+2.5},\fpeval{4.5+0.5}) {$t=2$};	
	\node[draw] at (\fpeval{\leftOffset+3.5},\fpeval{4.5+0.5}) {$t=3$};	
	\node[draw] at (\fpeval{\leftOffset+4.5},\fpeval{4.5+0.5}) {$t=4$};	
	\node at (\fpeval{\leftOffset+5.5},\fpeval{4.5+0.5}) {$\cdots$};	
	\node[draw] at (\fpeval{\leftOffset+6.5},\fpeval{4.5+0.5}) {$t=T$};
	\node at (\fpeval{\leftOffset+7.5},\fpeval{4.5+0.5}) {$\cdots$};
	\node[draw,align=right] at (\fpeval{\leftOffset+8.5+0.4},\fpeval{4.5+0.5}) {$t=T+2$};
	% additional vdots
	\node[left = 0cm of topd,align=left] at (\leftOffset,\fpeval{2.15}) {$\vdots$};
	\node at (\leftOffset+6,\fpeval{2.15}) {$\vdots$};
	% to highlight a specific point
	%\node at (0,0) [circle,fill,inner sep=1.5pt]{};
\end{tikzpicture}}
